Safe Policy Improvement by Minimizing Robust Baseline Regret

An important problem in sequential decision-making under uncertainty is to use limited data to compute a safe policy, i.e., a policy that is guaranteed to perform at least as well as a given baseline strategy. In this paper, we develop and analyze a new model-based approach to compute a safe policy when we have access to an inaccurate dynamics model of the system with known accuracy guarantees. Our proposed robust method uses this (inaccurate) model to directly minimize the (negative) regret w.r.t. the baseline policy. Contrary to the existing approaches, minimizing the regret allows one to improve the baseline policy in states with accurate dynamics and seamlessly fall back to the baseline policy, otherwise. We show that our formulation is NP-hard and propose an approximate algorithm. Our empirical results on several domains show that even this relatively simple approximate algorithm can significantly outperform standard approaches.

==> alternative.tex <==
\section{Alternative Bounds}

\subsection{An Alternative Bound on the Performance Loss of $\pi_{Ra}$}
\label{appendix:ThmPerfRewAdj2}

\begin{corollary}\label{coro:perf_reward_adjusted}
Given Assumption~\ref{asm:error}, the performance loss $\Phi(\pi_{Ra})$ also satisfies 
\[
\Phi(\pi_{Ra}) \le \min \left\{ \frac{\text{BR}(\pi_{Ra})}{1-\gamma}+\max_{\pi\in\Pi_S}\frac{2\gamma\rmax}{(1-\gamma)^2}  \| e_{\pi_{\widehat\M}} \|_{1,\pi^\pi_{\widehat\M}},  \Phi(\pi_B) \right\},
\]
where $\text{BR}(\pi_{Ra})=\max_{x\in\mathcal X}\left|\widehat{T}[\widehat{V}^{\pi_{Ra}}](x)-\widehat{V}^{\pi_{Ra}}(x)\right|$ is the Bellman residual w.r.t. Bellman operator $\widehat{T}[V](x)=\max_{a\in\mathcal A}\left\{\widehat r(x,a)+\gamma\sum_{x^\prime\in\mathcal X}\widehat{P}(x^\prime|x,a)V(x^\prime)\right\}$, value function $\widehat{V}^{\pi_{Ra}}(x)=\rho(\pi_{Ra},\widehat\M)$ at $x_0=x$ and $\pi^\pi_{\widehat\M}$ is the normalized state occupancy frequency of the policy $\pi$.
\end{corollary}

\begin{proof}%[Proof of Corollary \ref{coro:perf_reward_adjusted}]
Similar to the proof of  Theorem \ref{coro:perf_reward_adjusted}, we notice that
\begin{equation}\label{bdd:eval_sim}
\return(\pi^*_{\M^\star},\M^\star) - \return(\pi_0,\widetilde{\M}) =\underbrace{\return(\pi^*_{\M^\star},\M^\star)- \max_{\pi\in\Pi_S}\return(\pi,\widetilde{\M})}_{(a)} +\underbrace{\max_{\pi\in\Pi_S}\return(\pi,\widetilde{\M}) - \return(\pi_0,\widetilde{\M}) }_{(b)}
\end{equation}

First we prove an upper bound for (a). Recall the Bellman operator $\widehat T$ for value function $V:\reals^{\mathcal X}\rightarrow\reals^{\mathcal X}$ as $\widehat{T}[V](y)=\max_{a\in\mathcal A}\left\{\widehat r(y,a)+\gamma\sum_{y^\prime\in\mathcal X}\widehat{P}(y^\prime|y,a)V(y^\prime)\right\}$. Also define the value function $\widehat{V}^{\pi_0}(x)$ as $\return(\pi_0,\widetilde{\M})$ and the optimal value function $\widehat{V}(x)$ as $\max_{\pi\in\Pi_S}\return(\pi,\widetilde{\M})$, when the initial state is $x_0=x$. 
By applying the contraction mapping property on $\widehat{T} [\widehat{V}^{\pi_0}](y)-\widehat{V}^{\pi_0}(y)$ for any $y\in\mathcal X$ and combing with the definition of Bellman residual, one obtains
\[
\widehat{T}^2 [\widehat{V}^{\pi_0}](y)-\widehat{T}[\widehat{V}^{\pi_0}](y)\leq \gamma\text{BR}(\pi_0).
\]
By an induction argument, the above expression becomes 
\[
\widehat{T}^N[\widehat{V}^{\pi_0}](y)-\widehat{T}^{N-1}[\widehat{V}^{\pi_0}](y)\leq \gamma^{N-1}\text{BR}(\pi_0),
\]
for which by a telescoping sum, it further implies
\[
\widehat{T}^N [\widehat{V}^{\pi_0}](y)-\widehat{V}^{\pi_0}(y)= \sum_{k=1}^{N}\widehat{T}^k [\widehat{V}^{\pi_0}](y)-\widehat{T}^{k-1}[\widehat{V}^{\pi_0}](y)
\leq  \sum_{k=1}^N\gamma^{k-1}\text{BR}(\pi_0).
\]
By letting $N\rightarrow\infty$ and noticing that $\lim_{N\rightarrow\infty}\widehat{T}^N [\widehat{V}^{\pi_0}](y)=\widehat{V}(y)$, one finally obtains
\begin{equation}\label{eq:BR}
(b) \le\left|\max_{\pi\in\Pi_S}\return(\pi,\widetilde{\M}) - \return(\pi_0,\widetilde{\M})\right|=\left|\sum_{y\in\mathcal X} P_0(y)\left(\widehat{V}(y)-\widehat{V}^{\pi_0}(y)\right)\right|\leq  \lim_{N\rightarrow\infty}\sum_{k=1}^N\gamma^{k-1}\text{BR}(\pi_0)= \frac{\text{BR}(\pi_0)}{1-\gamma}.
\end{equation}
For an upper bound in (a), by interchanging $\M$ and $\widetilde\M$ in the derivation of \ref{eq:exp_proof_lower} and taking maximum on both sides, we also have,
\[
(a)=\max_{\pi\in\Pi_S}\return(\pi,{\M}^\star)-\max_{\pi\in\Pi_S}\return(\pi,\widetilde{\M})\le\max_{\pi\in\Pi_S}\frac{2\gamma\rmax}{1-\gamma} p_0\tr (\eye - \disc \widehat P_{\pi})^{-1} e_{\pi}\leq\max_{\pi\in\Pi_S}\frac{2\gamma\rmax}{(1-\gamma)^2}  \| e_{\pi_{\widehat\M}} \|_{1,\pi^\pi_{\widehat\M}} .
\]
Then the proof is completed by  combining both parts of the above arguments.
\end{proof}


\subsection{An Alternative Bound on the Performance Loss of $\pi_R$}
\label{appendix:ThmPerfRobust2}

\begin{corollary}\label{coro:perf_robust}
Given Assumption~\ref{asm:error}, the performance loss $\Phi(\pi_{R})$ also satisfies 
\[
\Phi(\pi_{R}) \le \min \left\{ \frac{\text{BR}(\pi_{R})}{1-\gamma}+\max_{\pi\in\Pi_S}\min_{P\in\mathcal{U}(\widehat{P},e)}\frac{2\gamma\rmax}{(1-\gamma)^2} \| e_{\pi_{\M(P)}} \|_{1,\pi_{\M(P)}},  \Phi(\pi_B) \right\},
\]
where $\text{BR}(\pi_{R})=\max_{x\in\mathcal X}\left|\mathcal{T}[{V}^{\pi_{R}}](x)-{V}^{\pi_{R}}(x)\right|$ is the Bellman residual w.r.t. Bellman operator $\mathcal{T}[V](x)=\max_{a\in\mathcal A}\left\{ r(x,a)+\gamma\min_{P\in\mathcal U(\widehat P,e)}\sum_{x^\prime\in\mathcal X}{P}(x^\prime|x,a)V(x^\prime)\right\}$, value function ${V}^{\pi_{R}}(x)=\min_{P\in\mathcal U(\widehat P,e)}\rho(\pi_{R},\M(P))$ at $x_0=x$ and $u^\pi_{\M(P)}$ is the normalized state occupancy frequency of the policy $\pi$.
\end{corollary}
\begin{proof}%[Proof of Corollary~\ref{coro:perf_robust}]
For the proof of the alternative performance bound, by following the same analysis as in the derivation of \eqref{bdd:eval_sim}, replacing the bellman operator $\widehat T$ with the robust Bellman operator:
\[
\mathcal{T}[V](y)=\max_{a\in\mathcal A}\left\{ r(y,a)+\gamma\min_{P\in\mathcal U(\widehat P,e)}\sum_{y^\prime\in\mathcal X}{P}(y^\prime|y,a)V(y^\prime)\right\},
\]
and defining the robust value function ${V}^{\pi_0}(x)$ as $\min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi_0,{\M}(P)\big)$ when the initial state is $x_0=x$,
we can easily show that
\[
\max_{\pi\in\Pi_S}\min_{P\in\mathcal{U}(\widehat{P},e)}\return(\pi,{\M}(P)) - \min_{P\in\mathcal{U}(\widehat{P},e)}\return(\pi_0,{\M}(P))\leq\frac{\text{BR}(\pi_0)}{1-\gamma},
\]
and
\[
\begin{split}
\max_{\pi\in\Pi_S}\return(\pi,{\M}^\star)-\max_{\pi\in\Pi_S}\min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi,\M(P)\big) \le&\max_{\pi\in\Pi_S}\min_{P\in\mathcal{U}(\widehat{P},e)}\frac{2\gamma\rmax}{1-\gamma} p_0\tr (\eye - \disc  P_{\pi})^{-1} e_{\pi}\\
\leq& \max_{\pi\in\Pi_S}\min_{P\in\mathcal{U}(\widehat{P},e)}\frac{2\gamma\rmax}{(1-\gamma)^2}  \| e_{\pi_{\M(P)}} \|_{1,u^\pi_{\M(P)}}.
\end{split}
\]
The proof is then completed by combining both of the above results.
\end{proof}

\subsection{An Alternative Bound on the Performance Loss of $\pi_{AR}$}
\label{appendix:robust_aug_perf2}

%Similar to Corollary \ref{coro:perf_robust}, we have the following result on an alternative performance bound that does not involve the optimal policy $\pi^*$. 

\begin{corollary}
\label{coro:perf_robust_aug}
Given Assumption~\ref{asm:error}, the performance loss $\Phi(\pi_{AR})$ also satisfies 
\[
\Phi(\pi_{AR}) \le \min \left\{ \frac{\text{BR}(\pi_{AR})}{1-\gamma}+\max_{\pi\in\Pi_S}\min_{P\in\mathcal{U}(\widehat{P},e)}\frac{2\gamma\rmax}{(1-\gamma)^2} \| e_{\pi_{\M(P)}} \|_{1,\pi_{\M(P)}},  \Phi(\pi_B) \right\}.
\]
where $u^\pi_{\M(P)}$ is the normalized state occupancy frequency of the policy $\pi$ and the Bellman residual for robust MDPs is $\text{BR}(\pi_{AR})=\text{BR}_{1,0}(\pi_{AR})$, for which the generic case $(\lambda_1,\lambda_2)\geq 0$, the Bellman residual w.r.t. Bellman operator $\mathcal{T}_{\lambda_1\lambda_2}[V](x,y)=\max_{a\in\mathcal A}\left\{ r^A_{\lambda_1,\lambda_2}(x,y,a)+\gamma\min_{P\in\mathcal U(\widehat P,e)}\sum_{x^\prime,y^\prime\in\mathcal X}{P}^A(x^\prime,y^\prime|x,y,a)V(x^\prime,y^\prime)\right\}$ is given by $\text{BR}_{\lambda_1,\lambda_2}(\pi_{RS})=\max_{x,y\in\mathcal X}\left|\mathcal{T}_{\lambda_1\lambda_2}[{V}_{\lambda_1\lambda_2}^{\pi_{AR}}](x,y)-{V}_{\lambda_1\lambda_2}^{\pi_{AR}}(x,y)\right|$ where ${V}^{\pi_{AR}}(x,y)=\min_{P\in\mathcal U(\widehat P,e)}\rho\big(\pi_{AR},\M^A_{\lambda_1\lambda_2}(P)\big)$ is the value function at $x_0=x$.
\end{corollary}

\begin{proof}
Since to the proof of Theorem~\ref{thm:perf_robust_aug}, the proof of this corollary follows identical arguments from Corollary~\ref{coro:perf_robust} and is omitted for the sake of brevity.
\end{proof}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%This lead to the primal Lagrangian formulation 
%%
%\begin{equation*}
%\max_{\pi\in\Pi_S^C} \min_{\lambda\geq 0}\min_{P\in\mathcal U(\widehat P,e)} L_P(\pi,\lambda)
%\end{equation*}
%%
%where $L_P(\pi,\lambda)$ is the Lagrangian function in \eqref{eq:lag}.
%
%Since $\pi_R\neq\pi_B$ is a safe policy and the feasible set $\mathcal C^{\text{robust}}$ is non-empty, the primal Lagrangian formulation implies $\max_{\pi\in\Pi_S^C} \min_{\lambda\geq 0}\min_{P\in\mathcal U(\widehat P,e)} L_P(\pi,\lambda)$ equals to the solution of \eqref{problem:ori}. Furthermore by weak duality, we have that 
%\[
%\max_{\pi\in\Pi_S^C} \min_{\lambda\geq 0}\min_{P\in\mathcal U(\widehat P,e)} L_P(\pi,\lambda) \leq  \underbrace{\min_{\lambda\geq 0}\max_{\pi\in\Pi_S^C}\min_{P\in\mathcal U(\widehat P,e)} L_P(\pi,\lambda)}_{\text{solution of Algorithm \ref{alg:robust_aug}} }.
%\] 
%
%On the other hand, consider the following maximization problem
%\begin{equation}\label{robust_pro_2}
%\max_{\pi\in \mathcal C^{\text{robust}}}\min_{\P\in\mathcal U(\widehat P,e)} \return( \pi,\M(P))
%\end{equation} 
%When $\pi_R\neq\pi_B$ is a safe policy, the feasible set $\mathcal C^{\text{robust}}$ is non-empty. Now let 
%\[
%L^R(\pi,\lambda)=\min_{\P\in\mathcal U(\widehat P,e)} \return( \pi,\M(P))+\lambda\left(\min_{\P\in\mathcal U(\widehat P,e)} \return( \pi,\M(P))-\return(\pi_B,\M^\star)\right)
%\]
%be the Lagrangian function for \eqref{robust_pro_2}. Since the feasible set is non-empty, we can drop the constraints in problem \eqref{robust_pro_2} and this problem is equivalent to
%\[
%\max_{\pi}\min_{\P\in\mathcal U(\widehat P,e)} \return( \pi,\M(P))
%\]
%where the dominating class of policies of this problem is stationary Markovian $\Pi_S$. Thus the primal Lagrangian duality formulation implies 
%\[
%\max_{\pi\in\Pi_S^C} \min_{\lambda\geq 0} L^R(\pi,\lambda)= \max_{\pi\in\Pi_S^C}\min_{P\in\mathcal U(\widehat{P})}\return(\pi,\M(P))=\max_{\pi\in\Pi_S}\min_{P\in\mathcal U(\widehat{P})}\return(\pi,\M(P)),
%\]
%i.e., $\max_{\pi\in\Pi_S^C} \min_{\lambda\geq 0} L^R(\pi,\lambda)$ equals to the solution of Algorithm \ref{alg:robust}.
%Since the objective function of \eqref{robust_pro_2} is lower than that of \eqref{problem:ori} and both problems share the same feasible set, it is obvious that 
%\[
%\max_{\pi\in\Pi_S^C} \min_{\lambda\geq 0}L^R(\pi,\lambda)\leq \max_{\pi\in\Pi_S^C} \min_{\lambda\geq 0}\min_{P\in\mathcal U(\widehat{P})}L_P(\pi,\lambda).
%\]
%
%Combining these arguments, we have just showed that if $\pi_R$ is a safe policy, then
%\[
%\return(\pi_B,\M^\star)\leq \min_{\mathcal P\in\mathcal U(\widehat{P})}\return(\pi_R,\M(P))\leq \min_{\lambda\geq 0}\max_{\pi\in\Pi_S^C}\min_{P\in\mathcal U(\widehat{P})}L_P(\pi,\lambda)\leq\min_{P\in\mathcal U(\widehat{P})} L_P(\pi_{RS},\lambda^*),
%\]
%where $(\pi_{RS},\lambda^*)$ is the \emph{minimax} saddle point solution of $\min_{P\in\mathcal U(\widehat{P})}L_P(\pi,\lambda)$.
%\end{proof}

==> approximate_models.tex <==
\newcommand{\polapprox}{\pi_{RaR}}

\section{Approximate Solutions}  \label{sec:SoluRobustBaseline}
In the previous section we illustrate two exact solution algorithms to problem \eqref{eq:objective_robust_interleave}. Unfortunately since this problem is NP-hard. Inherently the solution algorithms for robust policy improvement scale exponentially with the size of state and action spaces, which impedes the tractability of large scale implementation. To circumvent this issue, in this section, we propose several approximate solution algorithms and later compare their performance with the exact solution algorithm. 


\subsection{Solution for Sampled Model}

Before presenting any solution algorithms to guarantee safety, let us look at the naive approach of solving the simulated MDP $\widehat{\nat}$. Let $\polexp$ be an optimal policy for $\widehat{\nat}$:  $\polexp\in\argmax_{\pi\in\Polrand}\rho(\pi,\widehat{\nat}).$
The following theorem quantifies the performance loss of this policy.

\begin{theorem}  \label{thm:perf_naive}
	Let $\polexp$ be an optimal policy of the MDP $\widehat{\nat}$. Then under Assumption~\ref{asm:error}, the performance loss is bounded by
	\[
	\Phi(\polexp)\stackrel{\Delta}{=}\return(\pi^\star_{\nat\opt},\nat\opt) - \return(\polexp,\nat\opt) \le \frac{2 \gamma \rmax}{(1-\disc)^2}  \| e \|_\infty.  
	\]
\end{theorem}
The proof of this theorem follows the same lines of arguments of the performance analysis in Theorem \ref{thm:perf_robust_interleave} and can be found in the Appendix.
Unfortunately, there is no guarantee that $\polexp$ is \emph{safe}. Thus, deploying $\polexp$ may lead to undesirable outcomes due to model uncertainties. In the following section, we describe a method that can compute a safe policy and also provide better guarantees. 


\subsection{Robust MDP}\label{sec:robust}

In this section, we propose an algorithm for finding an approximated solution policy to problem \eqref{eq:objective_robust_interleave} via solving the robust MDP (RMDP). We prove that the policy returned by this algorithm is safe and has better (sharper) worst-case guarantees than the simulator based policy $\polexp$. 

\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Simulated MDP $\widehat{\nat}$, baseline policy $\pi_B$ and the error function $e$} 
\Output{Policy $\polrob$}
$ \pi_0 \leftarrow \argmax_{\pi\in\Pi_R} \min_{\nat\in\Nat}\rho\big(\pi,\nat\big)$ \;
$\rho_0 \leftarrow \min_{\nat\in\Nat} \rho\big(\pi_0,\nat\big)$ \; 
\leIf{$\rho_0 > \max_{\nat\in\Nat}\rho(\pi_B,\nat)$}{
$\polrob \leftarrow \pi_0$
}{
$\polrob \leftarrow \polbase$ \label{ln:algrob_condition}}
\Return $\pi_R$
\caption{Solution based on the RMDP} \label{alg:robust}
\end{algorithm}

The robust method makes use of the following approximation to the solution of problem \eqref{eq:objective_robust_interleave}:
\[
\begin{split}
&\max_{\pi \in\Pi_R} \min_{\nat\in\Nat} \Bigl( \return(\pi, \nat) - \return(\pi_B, \nat)\Bigr)\\
\geq& \max_{\pi \in\Pi_R} \min_{\nat\in\Nat} \return(\pi, \nat) -  \max_{\nat\in\Nat}\return(\pi_B, \nat)
\end{split}
\]
and guarantees safety by designing $\pi$ such that RHS of this inequality is always non-negative. 
Details of this methodology are summarized in Algorithm~\ref{alg:robust}. It first constructs and solves an RMDP. Then it returns its solution, if its worst-case performance over the uncertainty set is better than the robust performance $\max_{\nat\in\Nat}\rho(\pi_B,\nat)$, and returns $\pi_B$ otherwise. The following theorem shows that the policy $\pi_R$ is safe and quantifies its performance loss.  Details of this proof can be found in the Appendix.
\begin{theorem}\label{thm:perf_robust}
Given Assumption~\ref{asm:error}, the nonempty solution $\pi_R$ of Algorithm~\ref{alg:robust} is safe, i.e.,~$\rho(\pi_R,\nat\opt) \ge \rho(\pi_B,\nat\opt)$. Moreover, its performance loss $\Phi(\pi_R)$ satisfies
\[ 
\begin{split}
\Phi(\pi_R)\stackrel{\Delta}{=}&\return(\pi^\star_{\nat\opt},\nat\opt) - \return(\pi_R,\nat\opt) \\
 \le& \min \left\{\frac{2 \gamma \rmax}{(1-\disc)^2}  \| e_{\pi^\star_{\nat\opt}} \|_{1,u^\star_{\nat\opt}},\Phi(\pi_B)\right\}, 
 \end{split}
\]
where $u^\star_{\nat\opt}$ is the normalized state occupancy frequency of the optimal policy $\pi^\star_{\nat\opt}$ and $\Phi(\polbase)=\return(\pi^\star_{\nat\opt},\nat\opt) - \return(\polbase,\nat\opt)$ is the performance loss of the baseline policy.
\end{theorem}

Compared to $\Pi_R$ and the bound in Theorem~\ref{thm:perf_naive} on its performance loss, Theorem~\ref{thm:perf_robust} indicates that the policy $\pi_R$ returned by Algorithm~\ref{alg:robust} is safe and has a smaller bound on its performance loss. In particular, the bound depends only on a weighted $L_1-$norm of the errors for the optimal policy, instead of the $L_\infty-$norm over all policies. 

\subsection{Reward-adjusted MDP (RaMDP)}
Next we propose a method that relies on solving the simulator based MDP $\widetilde{\nat}=\langle\X,\A,\widehat{r},\widehat{P},p_0,\gamma\rangle\footnote{Here we overload the notation $\widetilde{\nat}$ to indicate the reward adjusted MDP, instead of a particular transition probability in $\Nat$.}$, which is exactly the same as the simulated MDP $\widehat{\nat}$, except that its reward function is \emph{adjusted} as $\widehat{r}(x,a)=r(x,a)-\frac{\gamma R_{\max}}{1-\gamma} e_P(x,a)$.
The unique property of this MDP is that, when Assumption~\ref{asm:error} holds, the performance of any policy $\pi$ in $\widetilde{\nat}$ is a lower-bound on its performance in the true MDP $\nat\opt$, i.e.,~$\rho(\pi,\widetilde{\nat})\le\rho(\pi,\nat\opt)$ (see Theorem~\ref{thm:perf_reward_adjusted}). 
Furthermore in comparison to the objective function of robust MDP, the following proposition shows that $\rho(\pi,\widetilde{\nat})$ is always a lower-bound of $\min_{\nat\in\Nat} \return\big(\pi,\nat\big)$.
\begin{proposition}
	\label{prop:robust-vs-rewad}
	Given Assumption~\ref{asm:error}, for each policy $\pi$, we have
	\[
	 \min_{\nat\in\Nat} \return\big(\pi,\nat\big) \ge \return(\pi,\widetilde{\nat}).
	\]
\end{proposition}
The proof of this proposition is given in the Appendix. Equipped with this result, one concludes that the reward-adjusted method approximates the solution of problem \eqref{eq:objective_robust_interleave} by inequality:
\[
\begin{split}
&\max_{\pi \in\Pi_R} \min_{\nat\in\Nat} \Bigl( \return(\pi, \nat) - \return(\pi_B, \nat)\Bigr)\\
\geq& \max_{\pi \in\Pi_R} \min_{\nat\in\Nat} \return(\pi, \nat)  -  \max_{\nat\in\Nat}\return(\pi_B, \nat)\\
\geq &\max_{\pi \in\Pi_R}  \return(\pi, \widetilde{\nat}) -  \max_{\nat\in\Nat}\return(\pi_B, \nat)
\end{split}
\]
and guarantees safety by designing $\pi$ such that RHS of this inequality is always non-negative. Algorithm~\ref{alg:reward-adjusted} summarizes the method for computing a policy using the reward adjusted MDP (RaMDP) $\widetilde{\nat}$. It returns an optimal policy of $\widetilde{\nat}$, when the performance of this policy in $\widetilde{\nat}$ is better than the baseline performance $\max_{\nat\in\Nat}\rho(\pi_B,\nat)$, and returns $\pi_B$ otherwise. 

\IncMargin{1em}
\begin{algorithm}
	\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
	\Input{Simulated MDP $\widehat{\nat}$, baseline policy $\pi_B$ and error function $e$} 
	\Output{Policy $\pi_{Ra}$}
	%\tcp{Compute $\widetilde{\nat}$ by adjusting the reward function of $\widehat{\nat}$ using~\eqref{eq:rhat}}
	$\widehat{r}(x,a) \leftarrow r(x,a)-\frac{\gamma R_{\max}}{1-\gamma} e_P(x,a)$ \;
	%\tcp{Solve the RaMDP $\widetilde{\nat}$}
	$\pi_0 \leftarrow \arg \max_{\pi\in\Pi_R} \rho(\pi,\widetilde{\nat})$ \;
	%\tcp{Compute the performance of $\pi_0$}
	$\rho_0 \leftarrow \rho(\pi_0,\widetilde{\nat})$ \;
	\leIf{$\rho_0 > \max_{\nat\in\Nat}\rho(\pi_B,\nat)$}{
		$\pi_{Ra} \leftarrow \pi_0$
	}{
	$\pi_{Ra} \leftarrow\pi_B$ \label{ln:algexp_condition}}
\Return $\pi_{Ra}$
\caption{Solution based on the RaMDP} \label{alg:reward-adjusted}
\end{algorithm}

Since the performance of any policy in $\widetilde{\nat}$ is a lower-bound on its performance in $\nat\opt$, it guarantees that the solution policy returned by Algorithm~\ref{alg:reward-adjusted}, $\pi_{Ra}$, performs at least as well as the baseline policy $\pi_B$. Theorem~\ref{thm:perf_reward_adjusted} shows that $\pi_{Ra}$ is a safe policy and quantifies its performance loss. 

\begin{theorem}\label{thm:perf_reward_adjusted}
	Given Assumption~\ref{asm:error}, the solution $\pi_{Ra}$ of Algorithm~\ref{alg:reward-adjusted} is safe, i.e.,~$\rho(\pi_{Ra},\nat\opt) \ge \rho(\pi_B,\nat\opt)$. Moreover, its performance loss $\Phi(\pi_{Ra})$ satisfies 
	\[ 
	\begin{split}
	\Phi(\pi_{Ra})\stackrel{\Delta}{=}&\return(\pi^\star_{\nat\opt},\nat\opt) - \return(\pi_{Ra},\nat\opt) \\
	 \le& \min\left\{\frac{2 \gamma \rmax}{(1-\disc)^2}  \| e_{\pi^\star_{\nat\opt}} \|_{1,u^\star_{\nat\opt}}, \Phi(\pi_{B})\right\},
	 \end{split}
	 \]
	where $u^\star_{\nat\opt}$ is the normalized state occupancy frequency of the optimal policy $\pi^\star_{\nat\opt}$ and $\Phi(\polbase)=\return(\pi^\star_{\nat\opt},\nat\opt) - \return(\polbase,\nat\opt)$ is the performance loss of the baseline policy.
\end{theorem}
Theorem~\ref{thm:perf_reward_adjusted}, whose proof is included in the Appendix, indicates that by this simple adjustment in the reward function of the simulated MDP $\widehat{\nat}$, we may guarantee that our solution is safe. Moreover, it shows that the bound on the performance loss of $\pi_{Ra}$ is actually tighter than that for the solution $\Pi_R$ of the simulator $\widehat{\nat}$ in Theorem~\ref{thm:perf_naive}. 

While the complexity of Algorithm \ref{alg:robust} is higher than that of Algorithm \ref{alg:reward-adjusted} (because solving RMDPs is more complex than standard MDP), Theorem~\ref{thm:perf_robust} does not show any advantage for $\pi_R$ over the policy $\pi_{RA}$ returned by Algorithm~\ref{alg:reward-adjusted}, neither in terms of safety nor in terms of the bound on its performance loss (Theorem~\ref{thm:perf_reward_adjusted}). 
On the other hand, while Algorithm~\ref{alg:reward-adjusted} guarantees to yield a safe policy is less complex than Algorithm~\ref{alg:robust}, from Proposition~\ref{prop:robust-vs-rewad} one notices that Algorithm~\ref{alg:reward-adjusted} may be overly conservative in many circumstances. 
This is because the adjustment of the reward function is based on the assumption that there exists a state with the optimal value of $\rmax / (1-\gamma)$ and that this state is accessible from each other state with the reward $\rmax$. This implies with extra computational complexity, the conservative-ness of safe policy search decreases.

%\subsection{Sub-optimality of Robust MDP Approximation}
%While the robust solution described in Algorithm~\ref{alg:robust} is less conservative than Algorithm~\ref{alg:reward-adjusted} it may nevertheless be overly restrictive. This is because the proposed improved policy $\pi_0$ is evaluated for the worst-case realization of the transition probability in $\Nat$ while the return of the baseline policy is with respect to $P\opt$. As a result, a candidate policy $\pi_0$ can be rejected even if for any realization $\nat\in\Nat$ the policy is better than the baseline. The aforementioned limitation as well as the the sub-optimal behavior of $\pi_R$ are illustrated in the following counter examples. This motivates our study of robust policy improvement in problem \ref{eq:objective_robust_interleave}, where such restriction is eliminated from the problem definition.
%
%\begin{example}
%The example in Figure~\ref{fig:conservative_joint} depicts the case in which the robust solution is too restrictive.
%\end{example}
%
%\begin{figure}[h]
%	\centering
%	\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.3cm,semithick]
%	\tikzstyle{action}= [circle,fill=black,text=white]
%	
%	\node[state] 		 (s1)                    														{$s_0$};
%	\node[action]      (a1)         [above right of=s1]     	{$a_1$};
%	\node[action]      (a2)         [below right of=s1]    {$a_2$};
%	
%	\node[state] (s2) [below right of=a1] {$s_1$};
%	
%	\node[action] (a11) [right of=s2,xshift=0mm] {$a_1$};
%	
%	\node (o1) [above right of=a11] {$+10$};
%	\node (o2) [below right of=a11] {$-10$};
%	
%	\path (s1) edge node [above left]{$\pi_{\text{B}}$}  (a1) ;
%	\path (a1) edge node[above right] {0} (s2);
%	\path (a11) edge node [above left]{$\xi^\star$} (o1);
%	\path (a11) edge node [below left]{$\xi_1$} (o2);
%	
%	\path (s1) edge node [below left]{$\pi^\star$}  (a2) ;
%	\path (a2) edge node[below right] {1} (s2);
%	
%	\path (s2) edge node[above] {$\pi^\star$} node[below] {$\pi_{\text{B}}$} (a11);
%	\end{tikzpicture}
%	\caption{Example in which the policy returned by~Algorithm~\ref{alg:robust} is too restrictive}
%	\label{fig:conservative_joint}
%\end{figure}
%\begin{figure}
%	\centering
%	\begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=1.3cm,semithick]
%	\tikzstyle{action}= [circle,fill=black,text=white]
%	
%	\node[state] 		 (s1)                    														{$s_0$};
%	\node[action]      (a1)         [above right of=s1]     	{$a_1$};
%	\node[action]      (a2)         [below right of=s1]    {$a_2$};
%	
%	\node (o11) [right of=a1] {$0$};
%	\node (o12) [right of=a2] {$10$};
%	
%	\node[state] (s2) [below right of=o11] {$s_1$};
%	
%	\node[action] (a11) [right of=s2,xshift=0mm] {$a_1$};
%	
%	\node (o1) [above right of=a11] {$+10$};
%	\node (o2) [below right of=a11] {$-10$};
%	
%	
%	\path (s1) edge node [above left]{$\pi_{\text{B}}$}  (a1) ;
%	
%	\path (a1) edge  (o11);
%	\path (a2) edge  (o12);
%	
%	\path (a11) edge node [above left]{$\xi^\star$} (o1);
%	\path (a11) edge node [below left]{$\xi_1$} (o2);
%	
%	\path (s1) edge node [below left]{$\pi^\star$} (a2) ;
%	
%	\path (s2) edge node[above] {$\pi^\star$} node[below] {$\pi_{\text{B}}$} (a11);
%	\end{tikzpicture}
%	 \caption{Example in which the policy returned by Algorithm~\ref{alg:robust} performs better than the baseline policy in some states but not in others.} 
%	 \label{fig:conservative_composed}
%\end{figure}
%
%\begin{example}
%Consider a simple MDP $\M$ is composed of two separate components $\nat_1$ and $\nat_2$ as depicted in Figure~\ref{fig:conservative_composed}. Suppose that the estimated model of $\nat_1$ is very good, while the model of $\nat_2$ is quite imprecise. Also assume that the initial distribution is uniformly distributed between an initial state in $\nat_1$ and an initial state in $\nat_2$. Intuitively, the best solution would use the optimized policy for $\nat_1$, which has a precise model, and use the baseline policy for $\nat_2$, which has an imprecise model. However, Algorithm~\ref{alg:robust} simply returns the baseline policy for both components because the return in $\nat_2$ potentially reduces the quality of the robust solution. It would beneficial in this case to combine the baseline policy with the optimized one instead of returning either one.
%\end{example}



==> bilinear_solution.tex <==
\subsection{The Surrogate Problem} \label{sec:surrogate}
Before getting into the policy optimization problem described in \eqref{eq:objective_robust_interleave}, we first consider the inner optimization problem in \eqref{eq:obj_interleave_inner} for any given policy $\pi\in\Pi_R$, namely $\min_{\xi\in\Nat}\return(\pi, \xi) - \return(\pi_B, \xi)$.
By Lemma 2 in \cite{Iyengar2005}, we show that this problem can indeed be re-cast as a bilinear optimization problem as follows:
\begin{align}
\min_{V_1,V_2,\,\,\nat\in\Nat}\,&\sum_{x}p_{0}(x) \left(V_1(x)+V_2(x)\right)\nonumber\\
\text{s.t.}\,&r_{\pi}(x)\!+\!\gamma\mathbb E_{\xi_{\pi}}[V_1\!\mid\! x]\leq V_1(x),\,\forall x.\nonumber\\
&-r_{\pi_B}(x)\!+\!\gamma\mathbb E_{\xi_{\pi_B}}[V_2\!\mid\! x]\leq V_2(x),\,\forall x.\nonumber
\end{align}
Here the rewards are given by $r_{\pi}(x)=\sum_{a}r(x,a)\pi(a|x)$, $r_{\pi_B}(x)=\sum_{a}r(x,a)\pi_B(a|x)$, and the transition probabilities are $\xi_{\pi}(x'|x)=\sum_{a}P(x'|x,a)\pi(a|x)$ and $\xi_{\pi_B}(x'|x)=\sum_{a}P(x'|x,a)\pi_B(a|x)$ respectively. 

While one can still compute the optimal policy using global optimization techniques such as branch and bound, due to the presence of bilinearity in $\mathbb E_{\xi_{\pi}}[V\!\mid\! x]$ and $\mathbb E_{\xi_{\pi_B}}[V\!\mid\! x]$ with respect to the terms $\pi$, $V_1$ and $V_2$, the solution algorithms are generally intractable. In the remaining part of this section, we aim to use McCormick's relaxation \cite{McCormick} to linearize the bilinear constraint. Immediately, we know that the solution to the problem with McCormick's relaxation is a lower bound to the inner optimization problem in \eqref{eq:obj_interleave_inner}.

Notice that by definition, we have $V_1(x,y)\in[-V_{\max},V_{\max}]$, for $V_{\max}=\frac{2R_{\max}}{1-\gamma}$. By the McCormick's envelope, the bilinear constraints $r_{\pi}(x)\!+\!\gamma\mathbb E_{\xi_{\pi}}[V_1\!\mid\! x]\leq V_1(x)$ and $-r_{\pi_B}(x)\!+\!\gamma\mathbb E_{\xi_{\pi_B}}[V_2\!\mid\! x]\leq V_2(x)$
can be approximated as follows:
\begin{equation}\label{constraints:Mccormick}
\begin{split}
&r_{\pi}(x)\!+\!\gamma\sum_{x'}\theta_1(x,x')\leq V_1(x),\\
&-r_{\pi_B}(x)\!+\!\gamma\sum_{x'}\theta_2(x,x')\leq V_2(x),\\
&\theta_1(x,x')\geq -V_{\max}\xi_{\pi}(x'|x),\,\theta_2(x,x')\geq -V_{\max}\xi_{\pi_B}(x'|x)\\
&\theta_1(x,x')\geq V_1(x')+V_{\max}\xi_{\pi}(x'|x)-V_{\max},\\
&\theta_2(x,x')\geq V_2(x')+V_{\max}\xi_{\pi_B}(x'|x)-V_{\max},\\
&\theta_1(x,x')\leq V_1(x') -V_{\max}\xi_{\pi}(x'|x)+ V_{\max},\\
&\theta_2(x,x')\leq V_2(x') -V_{\max}\xi_{\pi_B}(x'|x)+ V_{\max},\\
&\theta_1(x,x')\!\leq\! V_{\max}\xi_{\pi}(x'|x),\,\theta_2(x,x')\!\leq\! V_{\max}\xi_{\pi_B}(x'|x),\,\forall x,x',
\end{split}
\end{equation}
where $\theta_1(x,x')$ is the surrogate decision variable corresponding to the bilinear term $\xi_{\pi}(x'|x)V_1(x')$, and $\theta_2(x,x')$ is the surrogate decision variable corresponding to the bilinear term $\xi_{\pi_B}(x'|x)V_2(x')$. Here we also denote by $\Theta=[-2V_{\max},2V_{\max}]$ the feasible set for $\theta_1$ and $\theta_2$. Thus by applying the McCormick relaxation technique, we  obtain an approximate solution algorithm to problem \eqref{eq:objective_robust_interleave} that can be solved using linear programming techniques, such as the interior point method \cite{Bertsekas:NLP}.

Utilizing this result, we can show that the solution to the robust improvement problem in \eqref{eq:objective_robust_interleave} can be lower bounded by the solution of the following maximin problem:
\begin{align}
\max_{\pi\in\Pi_R}\,\,\min_{\theta_1,\theta_2\in\Theta,V_1,V_2,\,\,\nat\in\Nat}\,&\sum_{x}p_{0}(x) \left(V_1(x)+V_2(x)\right)\label{problem:maximin}\\
\text{s.t.}\,&\text{$(\pi,V_1,V_2,\theta_1,\theta_2,\nat)$ satisfies} \nonumber\\
&\text{the constraints in \eqref{constraints:Mccormick}.} \nonumber
\end{align}
Furthermore, by noticing that $\pi_B$ is a feasible solution of the above maximization problem whose solution is equal to zero, and by combining the lower bound property from McCormick's relaxation, the solution policy of the surrogate problem $\widetilde \pi^*$  is guaranteed to be \emph{safe}, i.e.,
\[
\min_{\xi\in\Nat}\return(\widetilde \pi^*, \xi) - \return(\pi_B, \xi)\geq 0.
\]
One way to compute the solution of the surrogate problem in \eqref{problem:maximin} is to replace the inner minimization problem with its dual. Parametrized by $\pi\in\Pi_R$, the inner problem is a linear program, thus strong duality holds. While its explicit representation is omitted in the main paper for the sake of brevity, the resultant maximization problem is still intractable for general problems, because the corresponding objective function is bilinear. Another method is to compute the parametrized solution of the inner problem using multi-parametric linear programming techniques \cite{MPT}, and to optimize the policy using global optimization methods such as coordinate descent \cite{CD} or  branch and bound \cite{BB}. 

In the rest of this section, we depict the following an iterative solution algorithm for the maximin problem. Consider the following policy improvement procedure:
\begin{itemize}
\item Initialize $\pi_0=\pi_B$.
\item Update the policy using the following expression:
\[
\pi_{k+1}=\mathcal P_{\Pi_R}\left\{\pi_k+\alpha_k \frac{F^*(\pi_k+\delta e)-F^*(\pi_k-\delta e)}{2\delta}\right\}
\] 
where $\delta>0$ is a discretization constant for the finite difference gradient approximation, $\mathcal P_{\Pi_R}$ is the Euclidean projection operator from $\reals^{|\mathcal X|\times|\mathcal A|}$ to $\Pi_R$, $\alpha_k$ is the step size which satisfies the following update rule: $\alpha_k>0$, $\sum_k\alpha_k=\infty$, $\sum_k\alpha_k^2<\infty$, and $F^*(\pi)$ is the optimal solution to the inner optimization problem in \eqref{problem:maximin} parametrized at policy $\pi$, i.e.,
\begin{align}
\min_{\theta_1,\theta_2\in\Theta,V_1,V_2,\,\,\nat\in\Nat}\,&\sum_{x}p_{0}(x) \left(V_1(x)+V_2(x)\right)\label{problem:maximin}\\
\text{s.t.}\,&\text{$(V_1,V_2,\theta_1,\theta_2,\nat)$ satisfies} \nonumber\\
&\text{the constraints in \eqref{constraints:Mccormick}.} \nonumber
\end{align}
\end{itemize}

Notice that at every given policy $\pi\in\Pi_R$, the inner optimization problem has a convex objective function and constraint. By the Envelop theorem of arbitrary sets \cite{}, we know that the gradient of $F^*(\pi)$ is given by the gradient of the objective function  in $\pi$, i.e., $\nabla_\pi\left[\sum_{x}p_{0}(x) (V^*_{1,\pi}(x)+V^*_{2,\pi}(x))\right]$, with respect to the following minimizers (parametrized in $\pi$) $\theta^*_1,\theta^*_2\in\Theta$, $V^*_1,V^*_2$, and $\nat^*\in\Nat$. Therefore as $\delta_k/\alpha_k\rightarrow 0$, the above policy improvement procedure resembles a SPSA based stochastic gradient ascent method, which converges to a local maxima $\pi^*$. Since the initial point is given by $\pi_B$, it guarantees that the policy $\pi^*$ is safe.





==> domains.tex <==
\section{Description of Experimental Domains} \label{app:domains}

\subsection{Grid Problem}  \label{app:grid_problem}

We now describe the grid problem in more detail. The state space in the problem comes from a two-dimensional grid: $\mathcal{S} = \{s_{ij} \ss i\in\mathcal{I}, j\in \mathcal{J}\}$; $i$ and $j$ represent a column and row respectively. Columns represent states of an interaction with the website, and rows represent more complex customer states, such as overall satisfaction. The dimensions are $|\mathcal{I}|= 12$ and $\mathcal{J}=3$.

There are 4 actions: $a_L$ for left, $a_R$ for right, $a_U$ for up, and $a_U$ for down. Rewards are independent of actions and depend only on states and only on the column: $x_{ij} = r_i$ where $r = [-1,1,2,3,2,1,-1,-2,-3,3,4,5]$. Actions left and right generally decrease and increase the column number; but can fail and in that case the transition is to a random column. The failure probability $z_j$ depends on the row $j$, with specific failure probabilities: $z=[0.9,0.2,0.3]$. If a transition fails, then the next state is chosen according to a fixed distribution which is generated a priori from a Dirichlet distribution. The distribution for first and last row are the same, and the middle row is the average of the two.

\cref{alg:transition} describes how the transition from a state is computed. The initial state is $s_{00}$.

\begin{algorithm}
	\KwData{Current state $s_{ij}$, action $a$, distributions $P_j$}
	\KwResult{Next state $s_{kl}$}
	
	\uIf{$\text{Random uniform from } [0,1] > z_j$}{
		\uIf{$a = a_R$}{
			$k \leftarrow i + 1$ \;
		}
		\uElseIf{$a = a_L$}{
			$k \leftarrow i - 1$ \;
		}
		\Else{
			$k \leftarrow \text{Random from } P_j$ \;
		}
		$k \leftarrow \max\{0, \min\{k, |\mathcal{I}|-1\} \}$ \;
	} 
	\Else{
		$k \leftarrow \text{Random from } P_j$ \;
	}
		
	\uIf{$a = a_U$}{
		$l \leftarrow j + 1$ \;
	}
	\uElseIf{$a = a_D$}{
		$l \leftarrow j - 1$ \;
	}
	\Else{
		$e \leftarrow \text{Random uniform from } [0,1]$ \;
		\uIf{$e \le 0.35$}{
			$l \leftarrow j + 1$ \;
		}
		\uElseIf{$e \le 0.7$}{
			$l \leftarrow j - 1$ \;
		}
		\Else{
			$l \leftarrow j$ \;
		}
	}
	$l \leftarrow \max\{0, \min\{l, |\mathcal{J}|-1\} \}$ \;
	\Return $s_{kl}$\;
	\caption{Transitions for state and action.} \label{alg:transition}
\end{algorithm}

\subsection{Energy Arbitrage} \label{app:energy_arbitrage}

The energy arbitrage model is based on \cite{Petrik2015}. We summarize it here for ease of reference. Recall that even though the state and action spaces in this problem are continuous, we discretize them as described in \cref{sec:experiments}.

The problem represents an energy arbitrage model with multiple finite \emph{known} price levels and a stochastic evolution given a limited storage capacity. In particular, the storage is assumed to be an electrical battery that degrades when energy is stored or retrieved.  Energy prices are governed by a Markov process with states $\Theta$. There are two energy prices in each time step: $p^i : \Theta \rightarrow \RealPlus$ is the purchase (or input) price and $p^o: \Theta \rightarrow \RealPlus$ is the sell (or output) price. Energy prices $\theta$ vary between 0 and 10 and their evolution is governed by a martingale with a normal distribution around the mean.

We use $s$ to denote the available battery capacity with $s_0$ denoting the initial capacity. The current state of charge is denotes as $x$ or $y$ and must satisfy that $0 \le x_t \le s_t$ at any time step $t$. The action is the amount of energy to charge or discharge, which is denoted by $u$. Positive $u$ indicates that energy is purchased to charge the battery; negative $u$ indicates the sale of energy. 

The battery storage degrades with use. The degradation is a function of the battery capacity when charged or discharged. We use a general model of battery degradation with a specific focus on Li-ion batteries. The degradation function $d(x,u) \in \RealPlus$ represent the battery capacity loss after starting at the state of charge $x \ge 0$ and charging (discharging if negative) by $u$ with $-x \le u \le s_0$.
This function indicates the loss of capacity, such that:
\[ s_{t+1} = s_t - d(x_t,u_t) \]

The state set in the Markov decision problem is composed of $(x,s,\theta)$ where $x$ is the state of charge, $s$ is the battery capacity, and $\theta\in\Theta$ is the state of the price process. The available actions in a state $(x,s,\theta)$ are $u$ such that $-x \le u \le s-x$. The transition is from $(x_t,s_t,\theta_t)$ to $(x_{t+1},s_{t+1},\theta_{t+1})$ given action $u_t$ is:
\begin{align*}
x_{t+1} &= x_t + u_t \\
s_{t+1} &= s_t - d(x_t,u_t)
\end{align*}
The probability of this transition is given by $P[\theta_{t+1} \vert \theta_t]$. The reward for this transition is:
\[ r((x_t,s_t,\theta_t), u_t) = \begin{cases} 
- u_t \cdot p^i - c^d \cdot d(x_t,u_t) &\text{if } u_t \ge 0 \\ 
- u_t \cdot p^o - c^d \cdot d(x_t,u_t) &\text{if } u_t < 0 \end{cases}.\]
That is, the reward captures the monetary value of the transaction minus a penalty for degradation of the battery. Here, $c^d$ represents the cost of a unit of lost battery capacity.

The Bellman optimality equations for this problem are:
\begin{equation}\label{eq:bellman_optimality_simple} 
\begin{aligned}
q_T(x,s,\theta) &= 0 \\
v_t(x,s,\theta_t) &= \min \bigl\{p^i_{\theta_t} \pos{u} + p^o_{\theta_t} \negt{u}  +  \\
& \quad + c^d \, d(x,u) +  \\
&\quad +q_t(x + u,s- d(x,u),\theta_t) :  \\
&\qquad :  u \in [ -x, s - x ] \bigr\}   \\
q_t(x , s, \theta_t) &= \lambda \cdot \operatorname{E}[v_{t+1}( x,s,\theta_{t+1}) ]
\end{aligned}
\end{equation}
where $\pos{u} = \max\{u, 0\}$ and $\negt{u} = \min\{u, 0\}$ and the expectation is taken over $P(\theta_{t+1} | \theta_t)$. 

Please see \cite{Petrik2015} for more details, including the price transition matrix. 


==> preamble.tex <==
\usepackage{color}
\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{graphicx}
\usepackage{comment,xspace}
%\usepackage{hyperref}
%\usepackage{algorithm,algorithmic} 
\usepackage{fancybox}

%\newcommand{\todo}[1]{\par\noindent{\color{red}\raggedright\sc{#1}
%    \par\marginpar{\Large \bf $\star$}}}

\newcommand{\D}{\displaystyle}
%%%%%
%% If you use a font encoding package, please enter it here, i.e.,
%  \usepackage{T1enc}

%% How many levels of section head would you like numbered?
%% 0= no section numbers, 1= section, 2= subsection, 3= subsubsection
%%==>>
\setcounter{secnumdepth}{3}

%%For margin comments
%\newcommand{\todomar}[1]{\marginpar{\tiny\color{red}#1}}
%% Math defs
\newcommand{\real}{{\mathbb{R}}}
\newcommand{\reals}{\real}
\newcommand{\sphere}{{\mathbb{S}}}
\renewcommand{\natural}{{\mathbb{N}}}
\newcommand{\naturals}{\natural}

\newcommand{\eps}{\varepsilon}
\newcommand{\He}{H_{\eps}}
\newcommand{\co}{\operatorname{co}}
\newcommand{\ov}{\overline}
\newcommand{\sign}{\operatorname{sign}}
\newcommand{\vers}{\operatorname{vers}}
\newcommand{\union}{\cup}

\newcommand{\map}[3]{#1: #2 \rightarrow #3}
\newcommand{\setdef}[2]{\left\{#1 \; | \; #2\right\}}
\newcommand{\until}[1]{\{1,\dots,#1\}}
\newcommand{\proj}[1]{\operatorname{proj}_{#1}}
\newcommand{\Ve}{\operatorname{Ve}}
\newcommand{\pder}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\tder}[2]{\frac{d #1}{d #2}}
%\newcommand{\margin}[1]{\marginpar{\tiny\ttfamily#1}}

\newcommand{\subscr}[2]{#1_{\textup{#2}}}

\newcommand{\TSP}{\ensuremath{\operatorname{TSP}}}
\newcommand{\MSP}{\ensuremath{\operatorname{MSP}}}
\newcommand{\MST}{\ensuremath{\operatorname{MST}}}
\newcommand{\OSS}{\ensuremath{\operatorname{OSS}}}
\newcommand{\sRH}{\textup{sRH}\xspace}
\newcommand{\mRH}{\textup{mRH}\xspace}
\newcommand{\mRHFG}{\textup{mRHFG}\xspace}

\newcommand{\card}{\operatorname{card}}
\newcommand{\E}[1]{\mathbb{E}\left[#1\right]}
\newcommand{\Vol}{\operatorname{Vol}}
\newcommand{\Area}{\operatorname{Area}}
\newcommand{\limn}{\lim_{n \rightarrow \infty}}
\newcommand{\limni}[1]{\lim_{n_{#1} \rightarrow \infty}}
\newcommand{\diam}{\operatorname{diam}}

%% theorems (always good to have some)
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{example}[theorem]{Example}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{assumption}[theorem]{Assumption}

%\newcommand{\proof}{\noindent{\bf Proof: \indent}}
%\newcommand{\proofover}{\hfill\vrule height8pt width6pt depth
%                0pt\newline}

\newcommand{\argmin}{\operatornamewithlimits{argmin}}
\newcommand{\reg}{$^{\textrm{\tiny\textregistered}}$}
\newcommand{\liml}{\lim_{\lambda \rightarrow +\infty}}



\newcommand{\prob}[1]{\mbox{$\mathbb{P}\left[#1\right]$}} 
\newcommand{\probnoarg}{\mbox{$\mathbb{P}$}} 
\newcommand{\expectation}[1]{\mbox{$\mathbb{E}\left[#1\right]$}} 
\newcommand{\probcond}[2]{\mbox{$\mathbb{P}\left(#1| #2\right)$}} 
\newcommand{\condexpectation}[2]{\mbox{$\mathbb{E}\left(#1| #2\right)$}} 
\newcommand{\iteratedexpectation}[2]{\mbox{$\mathbb{E}\left(\mathbb{E}\left(#1| #2\right)\right)$}} 



==> robust.tex <==
Robust optimization is a standard technique to deal with model uncertainty. In this section, we propose an algorithm for finding a safe policy via solving the robust MDP (RMDP). We prove that the policy returned by this algorithm is safe and has better (sharper) worst-case guarantees. 

\begin{algorithm}
\SetKwInOut{Input}{input}\SetKwInOut{Output}{output}
\Input{Simulated MDP $\widehat{\M}$, baseline performance $\rho(\pi_B,\M^\star)$ and the error function $e$} 
\Output{Policy $\pi_R$}
\tcp{Construct the uncertainty set}
$\mathcal U(\widehat{P},e)=\left\{ P ~:~ \| P(\cdot|x,a)-\widehat{P}(\cdot|x,a)\|_1\leq e(x,a), \; \forall x,a\in\mathcal{X}\times\mathcal{A} \right\} $ \;
%\tcp{Solve RMDP}
$ \pi_0 \leftarrow \argmax_{\pi\in\Pi_S} \min_{P\in\mathcal U(\widehat{P},e)}\rho\big(\pi,\M(P)\big)$ \;
$\rho_0 \leftarrow \min_{P\in\mathcal{U}(\widehat{P},e)} \rho\big(\pi_0,\M(P)\big)$ \; 
\leIf{$\rho_0 > \rho(\pi_B,\M^\star)$}{
$\pi_R \leftarrow \pi_0$
}{
$\pi_R \leftarrow \pi_B$ \label{ln:algrob_condition}}
\Return $\pi_R$
\caption{Solution based on the RMDP} \label{alg:robust}
\end{algorithm}

The robust method is summarized in \cref{alg:robust}. It first constructs an uncertainty set $\mathcal U(\widehat{P},e)$ using the simulator $\widehat{\M}$ and error function $e$. It then solves the resultant RMDP ($\M(P)$ with $P\in\mathcal U(\widehat{P},e)$) and returns its solution, if its worst-case performance over the uncertainty set is better than the baseline performance $\rho(\pi_B,\M^\star)$, and returns $\pi_B$ otherwise. 

\cref{alg:robust} involves solving a ($s,a$-rectangular) RMDP. RMDPs satisfy many of the same properties as regular MDPs, such as the existence of an optimal stationary policies.  RMDPs can often be solved quite efficiently by value iteration, policy iteration, or modified policy iteration~\cite{iyengar2005robust,kaufman2013robust,nilim2005robust,wiesemann2013robust}. In practical terms, solving an RMDP can be expensive due to the need to compute the worst-case transition probability which relies on solving a convex optimization problem for each state and action in every iteration. However, the robust solution can be computed very efficiently when the uncertainty set is described, as in our formulation, in terms of an $L_1$-norm~\cite{Petrik2015}; similar results also exist for the $L_2$ norm~\cite{iyengar2005robust}.
Since implementing \cref{alg:robust}  involves solving RMDPs, the complexity is $O(|\mathcal A||\mathcal X|^3\log(|\mathcal X|)/(1-\gamma))$ (for robust value iteration)~\cite{nilim2005robust}. It is higher than that in \cref{alg:reward-adjusted} but is still polynomial in $|\mathcal A|$, $|\mathcal X|$ and $1/(1-\gamma)$.  The following theorem shows that the policy $\pi_R$ is safe and quantifies its performance loss.  
\begin{theorem}\label{thm:perf_robust}
Given \cref{asm:error}, the nonempty solution $\pi_R$ of \cref{alg:robust} is safe, i.e.,~$\rho(\pi_R,\M^\star) \ge \rho(\pi_B,\M^\star)$. Moreover, its performance loss $\Phi(\pi_R)$ satisfies
\[ \Phi(\pi_R) \le \min \left\{\frac{2 \gamma \rmax}{(1-\disc)^2}  \| e_{\pi^\star_{\M^\star}} \|_{1,u^\star_{\M^\star}},\Phi(\pi_B)\right\}, \]
where $u^\star_{\M^\star}$ is the normalized state occupancy frequency of the optimal policy $\pi^\star_{\M^\star}$.
\end{theorem}
\begin{proof}%[Proof of Theorem~\ref{thm:perf_robust}]
To prove the safety of $\pi_R$ and bound its performance loss, we need to upper and lower bound the difference between the performance of any policy $\pi$ in the true MDP $\M^\star$ and its worst-case performance, $\min_{P\in\mathcal{U}(\widehat{P},e)} \return\big(\pi,\M(P)\big)$. Since $P^\star\in\mathcal{U}(\widehat{P},e)$ from Assumption~\ref{asm:error}, we have
%
\begin{equation} 
\label{eq:rob_proof_upper}
\min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi,\M(P)\big) \le \return(\pi,\M^\star).
\end{equation} 
%
Now let $\bar{P}$ be the minimizer in $\min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi,\M(P)\big)$. The minimizer exists because of the continuity and compactness of the uncertainty set. From Assumption~\ref{asm:error} and the construction of $\mathcal{U}(\widehat{P},e)$, for any $(x,a)\in\X\times\A$, we have
%
\begin{align*}
\| \bar{P}(\cdot|x,a) - P^\star(\cdot|x,a) \|_1 &\le \| \bar{P}(\cdot|x,a) - \widehat{P}(\cdot|x,a) + \widehat{P}(\cdot|x,a) + P^\star(\cdot|x,a) \|_1 \\
&\le \| \bar{P}(\cdot|x,a) - \widehat{P}(\cdot|x,a) \|_1 + \| \widehat{P}(\cdot|x,a) + P^\star(\cdot|x,a) \|_1  \\
&\le 2 e(x,a).
\end{align*}
%
Applying Lemma~\ref{lem:bound_transitions} with $\pi_1=\pi_2=\pi$, $\M_1=\M^\star$, and $\M_2=\M(\bar{P})$, we obtain
%
\begin{equation}
\label{eq:rob_proof_lower}
\return(\pi,\M^\star) - \min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi,\M(P)\big) \le \frac{2\gamma \rmax}{1-\gamma} \, p_0\tr (\eye - \gamma P^\star_\pi)^{-1}e_\pi = \frac{2\gamma \rmax}{(1-\gamma)^2} \, \| e_\pi \|_{1,u^\pi_{\M^\star}},    
\end{equation}
%
where $\pi^\pi_{\M^\star}= (1-\gamma) p_0^\top(\eye - \gamma P^\star_\pi)^{-1}$ is the normalized state occupancy frequency of policy $\pi$ in the true MDP $\M^\star$.

To prove the safety of the returned policy $\pi_{Ra}$, consider the two cases on Line~\ref{ln:algrob_condition} of Algorithm~\ref{alg:robust}. When the condition is satisfied, we have $\return(\pi_B,\M^\star)<\min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi_0,\M(P)\big)\leq\return(\pi_0,\M^\star)$, where the second inequality comes from~\eqref{eq:rob_proof_upper}, and thus, the policy $\pi_R=\pi_0$ is safe. When the condition is violated, then $\pi_R$ is simply $\pi_B$, which is safe by definition. 

To derive a bound on the performance loss of the returned policy $\pi_R$, consider also the two cases on Line~\ref{ln:algrob_condition} of Algorithm~\ref{alg:robust}. When the condition is satisfied, using~\eqref{eq:rob_proof_upper}, we have
%
\[ \Phi(\pi_R) = \return(\pi^\star_{\M^\star},\M^\star) - \return(\pi_0,\M^\star) \le \return(\pi^\star_{\M^\star},\M^\star) - \min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi_0,\M(P)\big)~, \]
%
and when the condition is violated, we have 
\[ \Phi(\pi_R) = \return(\pi^\star_{\M^\star},\M^\star) - \return(\pi_B,\M^\star)~. \]

Since the condition is satisfied on Line~\ref{ln:algrob_condition} of Algorithm~\ref{alg:robust} when $\min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi_0,\M(P)\big)>\return(\pi_B,\M^\star)$, we may write 
%
\[  \Phi(\pi_R) \le \min\left\{\return(\pi^\star_{\M^\star},\M^\star) - \min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi_0,\M(P)\big) ~ \return(\pi^\star_{\M^\star},\M^\star) - \return(\pi_B,\M^\star)\right\}~. \]
% 
Note that we may write the following inequalities for the first term in the minimum
\begin{align*}
\return(\pi^\star_{\M^\star},\M^\star) - \min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi_0,\M(P)\big) 
&\stackrel{\text{(a)}}{\leq} \return(\pi^\star_{\M^\star},\M^\star) - \min_{P\in\mathcal{U}(\widehat{P},e)}\return\big(\pi^\star_{\M^\star},\M(P)\big) \\
&\stackrel{\text{(b)}}{\le} \frac{2\gamma \rmax}{(1-\gamma)^2} \, \| e_{\pi^\star_{\M^\star}} \|_{1,u^\star_{\M^\star}},
\end{align*}
where {\bf (a)} follows from $\pi_0$ being the maximizer in solving the robust MDP, {\bf (b)} is from~\eqref{eq:rob_proof_lower} with $\pi=\pi^\star_{\M^\star}$, and $u^\star_{\M^\star}$ is the normalized state occupancy frequency of the optimal policy $\pi^\star_{\M^\star}$. 
\end{proof}


Compared to $\pi_S$ and the bound in \cref{thm:perf_naive} on its performance loss, \cref{thm:perf_robust} indicates that the policy $\pi_R$ returned by \cref{alg:robust} is safe and has a smaller bound on its performance loss. In particular, the bound depends only on a weighted $L_1-$norm of the errors for the optimal policy, instead of the $L_\infty-$norm over all policues. 

While the complexity of Algorithm \ref{alg:robust} is higher than that of Algorithm \ref{alg:reward-adjusted} (because solving RMDPs is more complex than standard MDP), \cref{thm:perf_robust} does not show any advantage for $\pi_R$ over the policy $\pi_{RA}$ returned by \cref{alg:reward-adjusted}, neither in terms of safety nor in terms of the bound on its performance loss (\cref{thm:perf_reward_adjusted}). This arises the question that why should one use the more complex \cref{alg:robust} in place of \cref{alg:reward-adjusted}. \cref{prop:robust-vs-rewadj} provides an answer to this question and shows whenever \cref{alg:reward-adjusted} returns a safe policy, so does \cref{alg:robust}, while the converse is not necessarily true. This implies with extra computational complexity, the conservatism of safe policy search decreases.

\begin{proposition}
\label{prop:robust-vs-rewadj}
Given \cref{asm:error}, for each policy $\pi$, we have
\[ \min_{P\in\mathcal{U}(\widehat{P},e)} \return\big(\pi,\M(P)\big) \ge \return(\pi,\widetilde{\M})~, \]
where $\widetilde{M}$ is defined in \cref{subsec:reward-adjusted}.
\end{proposition}
\begin{proof}
	Let $\bar{P}$ be the minimizer of $\min_{P\in\mathcal{U}(\widehat{P},e)} \return\big(\pi,\M(P)\big)$. Then from \cref{lem:bound_transitions} for each $\pi$:
	\begin{align*}
	\rho\big(\pi,\M(\bar{P})\big) \ge \rho(\pi,\widehat{\M}) - \frac{\gamma \rmax}{1-\gamma} p_0\tr (\eye - \gamma \widehat{P}_\pi)^{-1} e_\pi = \rho(\pi,\widetilde{\M}),
	\end{align*}
	The last inequality holds because $\widetilde{\M}$ is differs from $\widehat{\M}$ only in its reward function $\hat{r}^\pi=r^\pi-\frac{\gamma\rmax}{1-\gamma}e_\pi$ (see \eqref{eq:rhat}).
\end{proof}

Note that the bound in $\pi_R$ is based on the worst-case transition probabilities in $\mathcal U(\widehat{P},e)$. While this approach guarantees to yield a safe policy, it may still be too conservative as solving a RMDP considers finding a safe policy under the worst-case scenario. Next, we investigate an alternative approach to return a safe but less conservative policy.

%\begin{proof}
%To prove the safety of $\polrob$ and bound its performance loss, we will need to bound the approximated lower-bound return $\min_{P\in\mathcal{U}(\widehat{P})} \rho(\pi, P, r)$ in terms of the true return $\rho(\pi,P\opt,r)$ for any policy $\pi$. Since $P\opt \in \mathcal{U}(P)$ from \cref{asm:error} we have 
%\begin{equation} \label{eq:rob_proof_upper}
%\Bigl(\min_{P\in\mathcal{U}( \widehat{P} )}  \rho(\pi, P, r) \Bigr) - \rho(\pi, P\opt, r) \le 0 ~.
%\end{equation} 
%Now, let $\bar{P}$ be the minimizer in $\min_{P\in\mathcal{U}(\widehat{P})} \rho(\pi, P, r)$ (exists from continuity and compactness). Then from \cref{asm:error} and the construction of $\mathcal{U}(\widehat{P})$, we have:
%\begin{align*}
%\| \bar{p}(x,a) - p\opt(x,a) \|_1 &\le \| \bar{p}(x,a) - \widehat{p}(x,a) + \widehat{p}(x,a) + p\opt(x,a) \|_1 \\
%&\le \| \bar{p}(x,a) - \widehat{p}(x,a) \|_1 + \| \widehat{p}(x,a) + p\opt(x,a) \|_1  \\
%&\le 2 e(x,a) ~.
%\end{align*}
%Then, using \cref{lem:bound_transitions} with the above difference between $\bar{P}$ and $P\opt$,  we get:
%\begin{equation}\label{eq:rob_proof_lower}
%\Bigl(\min_{P\in\mathcal{U}( \widehat{P} )}  \rho(\pi, P, r) \Bigr) - \rho(\pi, P\opt, r) \ge - \frac{2\gamma \rmax}{1-\gamma} \, p_0\tr (\eye - P_\pi\opt ) \, e_\pi = - \frac{2\gamma \rmax}{(1-\gamma)^2} \, \| e_\pi \|_{1,u}  ~,    
%\end{equation}
%where $u_\pi$ is the normalized state occupancy frequency defined as:
%\[ u = (1-\gamma) (\eye - \gamma P_\pi\tr)^{-1} p_0. \]
%
%To prove the safety of $\polrob$, consider the two cases for the return of $\pi$  in \cref{ln:algrob_condition} of \cref{alg:robust}. When the condition is satisfied, then:
%\[ \return(\polbase, P\opt, r) < \min_{P\in\mathcal{U}(\widehat{P})} \return(\pi_0, P,r) \le \return(\pi_0, P\opt, r) \] 
%and therefore the policy $\pi_0$ is safe. When the condition is violated, then the returned policy is simply $\polbase$ which is safe by definition.
%
%Finally, we ready to show a bound on the performance loss of the computed policy. When the condition on \cref{ln:algrob_condition} is satisfied ($\min_{P\in\mathcal{U}(\widehat{P})} \return(\pi_0,P,r) > \return(\polbase,P\opt,r)$), then by \eqref{eq:rob_proof_upper} for $\pol_0$:
%\[ \Phi(\polrob) = \return(\pi\opt,P\opt,r) - \return(\pi_0,P\opt,r) \le \return(\pi\opt,P\opt,r) - \Bigl(\min_{P\in\mathcal{U}( \widehat{P} )}  \rho(\pi, P, r) \Bigr) ~,\]
%otherwise:
%\[ \Phi(\polrob) = \return(\pi\opt,P\opt,r) - \return(\polbase,P\opt,r).\]
%Observe that the condition is satisfied then the bound on the performance loss of $\pi_0$ is smaller than for the baseline policy and therefore we get
%\[ \Phi(\polrob) \le \min \, \Bigl\{  \return(\pi\opt,P\opt,r) - \Bigl(\min_{P\in\mathcal{U}( \widehat{P} )}  \rho(\pi, P, r) \Bigr) , \, \return(\pi\opt,P\opt,r) - \return(\polbase,P\opt,r) \Bigr\}~. \]
% Then by $\pi_0$ being the maximizer of $\min_{P\in\mathcal{U}( \widehat{P} )}  \rho(\pi, P, r)$ and by \eqref{eq:rob_proof_lower} applied to $\pi\opt$:
% \[ \return(\pi\opt,P\opt,r) - \Bigl(\min_{P\in\mathcal{U}( \widehat{P} )}  \rho(\pi, P, r) \Bigr) \le \return(\pi\opt,P\opt,r) - \Bigl(\min_{P\in\mathcal{U}( \widehat{P} )}  \rho(\pi, P, r) \Bigr) 
% \le \frac{2\gamma \rmax}{(1-\gamma)^2} \, \| e_\pi \|_{1,u} ~,\]
%where $u$ is the normalized occupancy frequency of $\pi\opt$. This proves the theorem.
%\end{proof}

%On the other hand, based on the structures of \cref{alg:expected} and \cref{alg:robust}, we immediately see that the computational complexity of  \cref{alg:expected} is less than the complexity of \cref{alg:robust}, because solving an MDP is easier than solving a RMDP. The following proposition, however, shows that the robust solution will always be at least as tight of a bound as the one with modified rewards. In addition, we show the robust bound can be significantly tighter than the one with adjusted rewards.
%
% 
%The advantage of using this methodology is that solving \cref{alg:robust} only involves a RMDP problem with $\mathcal X\times\mathcal A$ rectangular uncertainties. The theory behind this class of problems is well-studied in various literature~\cite{Iyengar2005,Nilim2005,Wiesemann2013}. The stationary Markov policy can be solved using robust value iteration, where each value iteration step involves a convex programming problem. However when the state and action spaces are large, solving this convex programming problem at each robust value iteration step could be expensive or even intractable. 
%
%Note that an s,a-rectangular MDP can be solved relatively efficiently in both theory and practice when the uncertainty set follows a certain structure. In particular, \cite{Petrik2015} describes and efficient method that eliminates the need for solving convex optimization problems in every update in the RMDP when the uncertainty set is described in terms on an $L_1$ norm. Similarly, \cite{Iyengar2005} shows similar results for both $L_1$ and $L_2$ norms.
%
%While \cref{alg:robust} does not have better guarantees on the performance loss than \cref{alg:expected}, the following proposition shows that the lower bound computed using the robust formulation is always at least as good as \cref{alg:expected}.
%
%\begin{proposition}
%\label{prop:robust-vs-rewadj}
%When \cref{asm:error} is satisfied then for each $\pi$:
%\[ \min_{P\in\mathcal{U}(\widehat{P})} \return(\pi,P,r) \ge  \return(\pi,\widehat{P},\widehat{r}) ~,\]
%where $\widehat{r}$ is defined as in \eqref{eq:rhat}.
%\end{proposition}
%\begin{proof}
%Let $\bar{P}$ be the minimizer of $\min_{P\in\mathcal{U}(\widehat{P})} \return(\pi,P,r)$. Then from \cref{lem:bound_transitions} for each $\pi$:
%\begin{gather*}
%\rho(\pi,\bar{P},r) \ge \rho(\pi,\widehat{P},r) - \frac{\gamma \rmax}{1-\gamma} p_0\tr (\eye - \gamma \widehat{P}_\pi)^{-1} e_\pi = \\
%= \rho\left(\pi, \widehat{P}, r- \frac{\gamma \rmax}{1-\gamma} e_\pi\right) = \rho(\pi,\widehat{P},\widehat{r})
%\end{gather*}
%This shows that the robust solution is never smaller than the one with adjusted rewards.
%\end{proof}
%
%\todo[author=Marek,inline]{Show also that there is an example in which the robust policy may work much better}
%
%Solving for $\polrob$ requires a worst-case policy search over all possible transition probabilities in $\mathcal U(\widehat{P})$. While $\polrob$ is guaranteed to be a safe policy, oftentimes it could be too conservative (i.e., results in a low long term discounted reward). In Section \ref{sec:aug_pol}, we will investigate an alternative methodology that returns a less conservative and safe policy.

